Rhythmic production of consonant-vowel syllables synchronizes traveling waves in speech-processing brain regions

Nature is abundant in oscillatory activity, with oscillators that have the remarkable ability of synchronizing to external events. Using electrocorticographic (ECoG) recordings from a subject rhythmically producing consonant-vowel syllables (CVSs) we show that neural oscillators recorded at individual ECoG electrodes become precisely synchronized to initiations of the production of CVSs (i.e., that these initiations occur at precise phases of bandpassed-filtered voltages recorded at most ECoG electrodes). This synchronization is not a trivial consequence of the rhythmic production of CVSs, since it takes several minutes to be fully established and is observed at the frequency of CVS production and at its second harmonic. The phase of filtered voltages at which CVSs are produced varies systematically across the grid of electrodes, consistently with the propagation of traveling waves (TWs). Using these synchronized phases we isolate a first TW in voltages (filtered at the median CVS-production frequency) moving from primary auditory to premotor cortex, and a second TW in high-gamma amplitude (coupled to phase at the CVS-production frequency) moving along the same path but in opposite direction. To our knowledge, this is the first report of rhythmic motor acts synchronizing spatio-temporally organized cortical activity in the human brain.

==> resultsSummary.tex <==

\subsection{Synchronization of neural populations to rhythmically produced CVSs}
\label{sec:syncInNeuralPopulations}

Here we demonstrate the synchronization of neural populations to rhythmically
produced \glspl{CVS} using recordings from electrode 136
(Figure~\ref{fig:grid}) in a \gls{CVS}-production session. In Section~\ref{sec:syncTWs} we describe this
synchronization across all electrodes in the grid. We first study
synchronization in oscillators running at the median \gls{CVS}-production
frequency (fundamental frequency; Section~\ref{sec:1-1SyncECoG}), and then in
oscillators running at the twice this frequency (second-harmonic;
Section~\ref{sec:2-1SyncECoG}).

\begin{figure}
\begin{center}
\includegraphics[width=6in]{figures/grid_layout_clipped.eps}
\end{center}

\caption{Grid of ECoG electrodes superimposed on an MRI reconstruction of the
subjects' brain.}

\label{fig:grid}
\end{figure}

\subsubsection{1-to-1 synchronization at the fundamental frequency}
\label{sec:1-1SyncECoG}

The black curve in Figures~\ref{fig:1-1SyncECoGBegining}
and~\ref{fig:1-1SyncECoGLater} plots voltages from electrode 136 bandpass
filtered around the median \gls{CVS}-production frequency at the beginning and
the middle of the \gls{CVS}-production session, respectively. Red vertical
lines mark times of initiation of \glspl{CVS} productions, and black vertical
lines mark peaks in voltage traces.
%
By the middle of the \gls{CVS}-production session
(Figure~\ref{fig:1-1SyncECoGLater}), but not at the beginning of this session
(Figure~\ref{fig:1-1SyncECoGBegining}), \glspl{CVS} initiations 
occur at precise times after filtered-voltage peaks (i.e.,
red vertical lines appear at similar delays after black vertical lines), and
filtered-voltage peaks and \gls{CVS} initiations are in a 1-to-1
correspondence (i.e., red vertical lines are matched to black vertical lines;
1-to-1 synchronization).

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{figures/EC2_B105/bpVoltagesWithCVSsElec136FPS762.94FromFreq0.40ToFreq0.80Order02FromTime000ToTime697_plotFromTime030ToTime040.eps}
\end{center}

\caption{At the beginning of the \gls{CVS}-production session, voltages from
electrode 136 filtered around the \gls{CVS}-production frequency are not
synchronized to \gls{CVS} initiations. The black trace plots the filtered
voltage, vertical black lines appear at peaks of the filtered voltage, and
vertical red lines indicate times of initiation of \gls{CVS} productions.}

\label{fig:1-1SyncECoGBegining}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{figures/EC2_B105/bpVoltagesWithCVSsElec136FPS762.94FromFreq0.40ToFreq0.80Order02FromTime000ToTime697_plotFromTime340ToTime350.eps}
\end{center}

\caption{Around 340~seconds into the \gls{CVS}-production session almost
perfect synchronization is achieved between \glspl{CVS} initiations and
voltages from electrode 136 filtered around the median \gls{CVS}-production
frequency.
The black trace plots the filtered
voltage, vertical black lines appear at peaks of the filtered voltage, and
vertical red lines indicate times of initiation of \gls{CVS} productions.}

\label{fig:1-1SyncECoGLater}
\end{figure}

\subsubsection{2-to-1 synchronization at the second harmonic}
\label{sec:2-1SyncECoG}

We bandpass filtered the
\gls{ECoG} recordings around the second \gls{CVS}-production frequency harmonic.
Figures~\ref{fig:2-1SyncECoGBegining} and~\ref{fig:2-1SyncECoGLater} are as
Figures~\ref{fig:1-1SyncECoGBegining} and~\ref{fig:1-1SyncECoGLater}, but for
voltages filtered around the second \gls{CVS}-production frequency harmonic.
Again we see that around 345~seconds in the \gls{CVS}-production session
(Figure~\ref{fig:2-1SyncECoGLater}), but not at the beginning of this session
(Figure~\ref{fig:2-1SyncECoGBegining}), the filtered-voltage
oscillations are precisely synchronized to the initiations of \gls{CVS}.
Figure~\ref{fig:2-1SyncECoGLater}
shows that each other oscillation is synchronized to the initiation of a
\gls{CVS} (i.e., 2-to-1 synchronization).

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{figures/EC2_B105/bpVoltagesWithCVSsElec136FPS381.47FromFreq1.00ToFreq1.40Order03FromTime000ToTime697_plotFromTime030ToTime040.eps}
\end{center}

\caption{At the beginning of the \gls{CVS}-production session no synchronization
is apparent between \gls{CVS} initiations and peaks of voltages from electrode 136 filtered around
the second harmonic of the \gls{CVS}-production frequency. Same format as in
Figure~\ref{fig:1-1SyncECoGBegining}.}

\label{fig:2-1SyncECoGBegining}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=3.5in]{figures/EC2_B105/bpVoltagesWithCVSsElec136FPS381.47FromFreq1.00ToFreq1.40Order03FromTime000ToTime697_plotFromTime340ToTime350.eps}
\end{center}

\caption{By 340 seconds into the \gls{CVS}-production session an almost perfect
synchronization develops between the initiation of \glspl{CVS} and voltages
from electrode 136 filtered around the second harmonic of the median
\gls{CVS}-production frequency. The synchronization is 2-to-1 (two
filtered-voltage oscillations are paired with one \gls{CVS} initiation). Same
format as in Figure~\ref{fig:1-1SyncECoGLater}. The green vertical lines
mark peaks of filtered voltages not paired to \gls{CVS} initiations.}

\label{fig:2-1SyncECoGLater}
\end{figure}

\subsection{Synchronization of traveling waves to rhythmically produced
consonant-vowel syllables}
\label{sec:syncTWs}

The previous section showed that \glspl{cvsPhase} of voltages from electrode
136 were highly concentrated.
%
Section~\ref{sec:cvsPhaseaAcrossElectrodes} below demonstrates that this high
concentration extends across most electrodes in the grid, and shows that
\glspl{cvsPhase} are spatially organized consistently with the propagation of
\glspl{TW}.
%
Using this spatial organization, Section~\ref{sec:a1PremotorTWs} isolates an
extended \gls{TW} in voltages filtered around the median \gls{CVS}-production
frequency moving from primary auditory cortex to premotor cortex, and a
\gls{TW} in coupled high-gamma amplitude moving along the same path \gls{TW}
but in opposite direction.

\subsubsection{Synchronization of oscillators across electrodes}
\label{sec:cvsPhaseaAcrossElectrodes}

Figure~\ref{fig:cvsPhasesAllElectrodesManyTWs} shows histograms of
\glspl{cvsPhase} for voltages filtered around the median \gls{CVS}-production
frequency between 340 and 400~seconds of the \gls{CVS}-production session.
%
In those histograms with high concentration of \glspl{cvsPhase} (i.e.,
\gls{PLI}\textgreater 0.5), a red segment indicates the mean phase (i.e., mean
direction, Section~\ref{sec:circularStats}).
%
In most
histograms the distribution of \glspl{cvsPhase} is highly concentrated
and
their mean phase orderly shifts from one electrode to its
neighbors (i.e., red segments change smoothly across the electrode grid).

The mean \gls{cvsPhase} should decrease as we move from one electrode
to the next along the propagation direction of a \gls{TW}. That is, in the
\gls{cvsPhase} histograms the red segment should move clockwise as we move
along the direction of propagation of a \gls{TW}. The yellow arrows in
Figure~\ref{fig:cvsPhasesAllElectrodesManyTWs} join neighboring histograms with
a high \gls{cvsPhase} concentration and
point in the direction consistent with the propagation of a \gls{TW}.

Histograms with a high \gls{cvsPhase} concentration are located in primary
auditory cortex (bottom right), in the ventral sensorimotor cortex (center
middle), and in the premotor cortex (top left) and \glspl{TW} can be found
between these areas, as illustrated next.

\begin{figure}
\begin{center}
\includegraphics[width=7.0in,angle=0]{figures/EC2_B105/histCVSPhasesFPS762.94FromFreq0.40ToFreq0.80FromTime340ToTime400ITCThr0.50_manyTWs.eps}

% \captionof{figure}{%
\caption{
% 
Histograms of \glspl{cvsPhase} for all electrodes in the grid.
%
Red segments are drawn at the mean \gls{cvsPhase} (mean direction,
Section~\ref{sec:circularStats}) in histograms with high \gls{cvsPhase}
concentration (\gls{PLI}\textgreater 0.5, Section~\ref{sec:circularStats}).
%
\glspl{cvsPhase} should decrease between one electrode and the next along the
direction of propagation of a \gls{TW} (i.e., red segments should move in the
clockwise direction).
%
Yellow arrows joining neighbor electrodes point in the direction consistent
with the propagation of a \gls{TW}.
%
The title of each histogram gives the electrode number, the \gls{PLI}, and the
p-value of a Rayleigh non-uniformity test. 
%
Histograms with high concentration of \glspl{cvsPhase} are mostly located in
the auditory cortex (bottom right), ventral sensorimotor cortex (center
middle), and premotor cortex (top left), and \glspl{TW} can be found between
some of these areas (e.g., Section~\ref{sec:a1PremotorTWs}).
%
}

\label{fig:cvsPhasesAllElectrodesManyTWs}
\end{center}
\end{figure}

\subsubsection{TWs between premotor and primary auditory cortex synchronized to
the production of CVSs}
\label{sec:a1PremotorTWs}

The video at \url{https://youtu.be/CkQCau8RKvI} depicts a \gls{TW} moving from
primary auditory to premotor cortex.


Using the same recordings as those characterized here, in
\citet{rapelaInPrepTWsInSpeech} we reported \glspl{TW} in voltages filtered
around the median \gls{CVS}-production frequency and described a peculiar
organization of the coupling between phases of the filtered voltages and
high-gamma amplitudes.  We showed that this phase-amplitude coupling led to
\glspl{TW} of coupled high-gamma amplitude moving along the same path, but in
opposite direction, as \glspl{TW} of voltages filtered around the median
\gls{CVS}-production frequency.
%
The video at \url{https://youtu.be/8pdl6i7jnbw} shows a TW of coupled
high-gamma amplitude moving in the opposite direction as the \gls{TW} shown in
the previous video.
%
Both \glspl{TW} were extracted from a middle section of the \gls{CVS}-production
session (between 340 and 400~seconds from the start of the session).

It took several minutes from the start of the \gls{CVS}-production session for
the establishment of \glspl{TW}. The videos at
\url{https://youtu.be/NDrmVZ9lg9E} and at \url{https://youtu.be/n_4KWWrKfBQ}
show voltages filtered around the median \gls{CVS}-production frequency and
coupled high-gamma amplitudes, respectively, extracted from the initial section
of the \gls{CVS}-production section. \glspl{TW} in this initial section are
weaker than those in the middle section of this session.


